QPRAC: Towards Secure and Practical PRAC-based Rowhammer Mitigation using Priority Queues

JEDEC has introduced the Per Row Activation Counting (PRAC) framework for DDR5 and future DRAMs to enable precise counting of DRAM row activations. PRAC enables a holistic mitigation of Rowhammer attacks even at ultra-low Rowhammer thresholds. PRAC uses an Alert Back-Off (ABO) protocol to request the memory controller to issue Rowhammer mitigation requests. However, recent PRAC implementations are either insecure or impractical. For example, Panopticon, the inspiration for PRAC, is rendered insecure if implemented per JEDEC's PRAC specification. On the other hand, the recent UPRAC proposal is impractical since it needs oracular knowledge of the `top-N' activated DRAM rows that require mitigation. This paper provides the first secure, scalable, and practical RowHammer solution using the PRAC framework. The crux of our proposal is the design of a priority-based service queue (PSQ) for mitigations that prioritizes pending mitigations based on activation counts to avoid the security risks of prior solutions. This provides principled security using the reactive ABO protocol. Furthermore, we co-design our PSQ, with opportunistic mitigation on Refresh Management (RFM) operations and proactive mitigation during refresh (REF), to limit the performance impact of ABO-based mitigations. QPRAC provides secure and practical RowHammer mitigation that scales to Rowhammer thresholds as low as 71 while incurring a 0.8% slowdown for benign workloads, which further reduces to 0% with proactive mitigations.

==> outline.tex <==

\section{Flow -- (To be removed)}
\hfill \break
\underline{High Level Story:}
\begin{itemize}
    \item \textbf{PRAC is proposed in DDR5 Spec}. A couple of implementations have emerged.
    \item \textbf{We show that existing implementations are either not secure or not practical.} JEDEC PRAC spec guarantees neither, it is just a contract. 
    \item \textbf{We propose the first PRAC implementation in DRAM that is both secure and practical using priority queues for mitigation.} 
    \begin{itemize}
        \item We provide queue size constraints, insertion policy, eviction policy, mitigation policy (when to raise ALERT) for this priority queue implementation.   
        \item We provide a security bound for the maximum disturbance given a certain ALERT back off threshold and ALERT-RFM and ALERT-ALERT delays, and propose what the ALERT threshold should for different TRH to be secure.
        \item We measure the performance impact vs TRH. (\TODO{This should be possible to evaluate with DRAMSec paper's simulator}).
    \end{itemize}
    
    \item \textbf{What about performance attacks?} Thus far, we have analyzed PRAC as the first line of defense. This makes it considerably vulnerable to performance attacks.
    \begin{itemize}
        \item We propose proactively mitigating the highly activated rows. \TODO{We can evaluate memory performance attack vs TRH, for PRAC.} 
        %\hl{PN -- \emph{I do not think we should call it PRIDE. The proactive defence uses count values to determine probabilities, so it isn't PRIDE}.}
        \item We can use the priority queue itself to make proactive mitigations at tREFI. Queue size determines how useful proactive mitigations are, and impacts number of reactive ALERTs needed. \TODO{Need to evaluate how good this hybrid implementation performs for benign and performance attack workloads.}
    \end{itemize}
    
    \item \textbf{Conclusion: First secure and practical PRAC implementation.} Bonus: We provide hybrid of proactive (trefi) and reactive (PRAC) in-DRAM defenses more resilient to performance attacks than only PRAC.
    
\end{itemize}

\hfill \break
\underline{Drawbacks of Prior Work.}
\begin{itemize}
    \item \textbf{Insecurity of Panopticon Design}
    \begin{itemize}
        \item Whenever the \textbf{threshold bit} is toggled during a counter increment, Panopticon enqueues the row address into a mitigation service queue. When queue is full, it raises ALERT. 
        \item This is unsafe if the ALERT is non-blocking. For example, queue is full and additional activations cause entries to get evicted. The same row will be re-inserted only after $2^\textbf{threshold-bit}$ activations.
    \end{itemize}
    \item \textbf{UPRAC Needs Queue for Practical Implementation}
    \begin{itemize}
        \item \textbf{Impractical assumption that top-K activated rows can be identified} and mitigated, when ALERT is issued. Alert is issued when a single counter crosses back off threshold. Searching through DRAM for identifying the top-K rows is not practical, without maintaining some queues. Implementations of these queues themselves can introduce vulnerabilities.
        \item \textbf{FIFO Service Queue like Panopticon is Insecure.}
        %Size vs tABO\_ACT and tABO\_Delay}:
        After triggering an ALERT (non-blocking), we have tABO\_ACT to continue filling the queue, and tABO\_Delay ACTs between two ALERTS. Given N\_mit = tABO\_Delay, We can refill the queue at a greater rate (tABO\_ACT + tABO\_Delay) than we can remove from the queue (N\_mit). Thus, a simple queue can easily overflow, and we can deterministically force some rows to be evicted from queues and not be mitigated.
%         \textbf{Personal note To-Be-Confirmed}: You can       technically never match the insertion rate, even with blocking ALERT\_n. Assuming blocking and $|Q|$ is the current queue occupancy when an ACT triggers the ALERT\_n, the occupancy is $|Q| + 1$. Then, N\_ref rows are refreshed. However, since tABO\_Delay = N\_ref, we can fill the queue back to $|Q| + 1$. The next ACT after tABO\_Delay, as per the spec, can trigger another ALERT\_n, which causes the queue to fill to $|Q| + 2$.\\
    \end{itemize}
\end{itemize}

\hfill \break
\underline{Proposed Solution-1: Practical and Secure PRAC.}

\begin{itemize}
    \item We propose to make UPRAC's assumption of mitigating the
    highest count practical using a priority queue. 
    \item \textbf{Priority queue design}. Has entries with RowID and ACT-count. Size is greater or equal to N\_mit. We insert a row into the queue if it has a PRAC count higher than the entry with minimum count and evict min count entry. 
    \item \textbf{Mitigation Policy.} Top N\_mit entries by count values will get mitigation  on ALERT. ALERT raised when even one entry crosses ALERT threshold (similar to UPRAC).
    %We need to size this queue to be greater or equal to N\_ref and setting the threshold level (100, 90, 80, 70\%) to the appropriate percentages. 
    \item \textbf{Security Guarantee.} We can bound the amount of ACT above the ALERT threshold level similar as the wave attack in UPRACT, except there will be a additive correction factor of {tABO\_ACT + tABO\_Delay}, due to the queue eviction.
    \item \textbf{Performance against Benign and Degradation Attack}: We show with result whether the performance on these workloads remains similar to what UPRAC theorized. This lays out the problem of performance attacks, that we propose to fix using hybrid designs. \TODO{evals in UPRAC's Simulator}
\end{itemize}

\hfill \break
\underline{Proposed Solution-2: PRAC Resilient to Performance Attack.}
\begin{itemize}
    \item \textbf{Naive Solution is Not the Best.} Proactively draining the top activation count row on tREFI, may not be the most optimal (easily leveraged in performance attack).
    \item \textbf{Proposal - Probabilistic Mitigation}: Use the entries in the priority queue for mitigation, on tREFI, probabilistically. This enables the overall number of ALERTs to be reduced, or atleast not be as bunched up.
       
%    To be honest, I am a little foggy about how we are getting the rows well below the threshold level. The main idea from what I remember was to find time in either periodic refreshes in between tREFis or randomly mitigate rows in the queue.
    \begin{itemize}
        \item \TODO{Evaluations}: Evaluate Effect of Degradation attack (Should be less compared to Proposal-1 (Reactive alone) or Proposal-2A (PRIDE + PRAC), as TRH drops.)
        \item Evaluate Performance impact on benign applications.
        \item Evaluate Storage.
        \item Evaluate Energy.
    \end{itemize}    
    
\end{itemize}
